DNA-Based Storage: Models and Fundamental Limits

Due to its longevity and enormous information density, DNA is an attractive medium for archival storage. In this work, we study the fundamental limits and trade-offs of DNA-based storage systems by introducing a new channel model, which we call the noisy shuffling-sampling channel. Motivated by current technological constraints on DNA synthesis and sequencing, this model captures three key distinctive aspects of DNA storage systems: (1) the data is written onto many short DNA molecules; (2) the molecules are corrupted by noise during synthesis and sequencing and (3) the data is read by randomly sampling from the DNA pool. We provide capacity results for this channel under specific noise and sampling assumptions and show that, in many scenarios, a simple index-based coding scheme is optimal.

==> achievability.tex <==
% !TEX root = DNA_storage_main.tex


Suppose we use the first $\log \M$ bits in each molecule to encode a distinct tag for each molecule.
Then we have $\len - \log \M = \len(1 - 1/\beta)$ symbols per molecule to encode data, and the channel effectively becomes an erasure channel where each symbol (i.e., each molecule) is erased with probability $(1 - 1/\M)^{\M \cNM}$. 
The storage rate $R_s$ achieved is thus $(1-e^{-\cNM})(1-1/\beta)$ (recall that $\lim_{\M\to\infty} (1 - 1/\M)^{\M \cNM} = e^{-\cNM}$). 
%, which agrees with the information theoretic bound in Theorem 1.


%\aln{
%\left( \left| \{ i : \
%}


==> poisson_channel.tex <==
% !TEX root = DNA_storage_journal_v2.tex



\subsection{Poisson channel}

\mycomment{Discuss - do we want to include something from this? Does not have high priority, but perhaps for a future version.}


In the error-free case, the DNA storage channel can be seen as channel over the $|\Sigma^L|$ distinct strings that can be written into the channel.
When viewed this way, the input to the channel is 
the number of copies of a given string in $t \in \Sigma^L$, and the output is the number of such strings that are sampled.
Since the number of times a given molecule is sampled can be well approximated by a Poisson random variable with mean $c = N/M$, the channel can then be described (or in fact defined) as
\al{
x[t] \in \Z^+ \quad \longrightarrow \quad  y[t] \sim \Pois(cx[z]),
}
for $t \in \Sigma^L$.
Since we are only allowed to write $M$ molecules, and if we assume the binary case for simplicity, we have the ``average power'' constraint 
\aln{
\sum_{t\in \Sigma^L} x[z] \leq M \,  \Leftrightarrow \, E\left(x[t]\right) \leq \frac{M}{2^L} = M^{1-\beta},
}
where we let $L = \beta \log M$.

The regime we had previously considered, with $\beta > 1$, corresponds to a Poisson channel in which the power goes to zero as the blocklength goes to infinity.
In the regime $\beta < 1$, on the other hand, the power is going to infinity, and looking at the DNA storage channel as a Poisson channel seems reasonable.

In fact, \cite{LapidothPoisson} provides the following result about the capacity of a Poisson channel:

\begin{theorem}
Consider the Poisson channel
\al{
x[t] \geq 0 \quad \longrightarrow \quad  y[t] \sim \Pois(x[t]),
}
with average power constraint $E\left(x[t]\right) \leq P$. The capacity $C(P)$ satisfies 
\aln{
\lim_{P \to \infty} \left( C(P) - \frac12 \log P \right) = 0.
}
\end{theorem}


\mycomment{
What does this result give? 
We have $2^L$ channel uses, as this is the number of different fragments. 
The number of bits per nucleotide is then:
\[
\frac{2^\len}{\len \M} \frac{1}{2} \log(P)
=
\frac{\M^\beta}{\beta \log(\M) \M} \frac{1}{2} \log(\M) (1-\beta)
=
\frac{1 - \beta}{2\beta} \M^{-(1-\beta)}.
\]
This is exactly the same number as we obtained from the counting argument in~\eqref{eq:capboundcount} (up to the factor of two, which might be a error ?
}







A consequence of this result is that, for a Poisson channel where the power constraint grows with the blocklength, the maximum achievable normalized rate is characterized:

\begin{definition}
Consider the Poisson channel 
\aln{
x[t] \geq 0 \quad \longrightarrow \quad  y[t] \sim \Pois(x[t]), 
}
with power constraint $\tfrac1n\sum_{t=1}^n x[t] \leq n^\alpha$.
We refer to this channel as the Poisson channel with increasing power (PCIP).
We say that $\rho > 0$ is an achievable normalized rate if, for every $\ep > 0$, one can design a code 
 for some blocklength $n$ with error probability at most $\ep$ and rate $\rho \log n$.
 Let $\bar C(\alpha)$ be the closure of achievable normalized rates.
\end{definition}

\begin{conjecture}
For the PCIP, $\bar C(\alpha) = \alpha/2$.
\end{conjecture}

\begin{proof}
\emph{Achivability: }\;
Take any $\rho < \alpha/2$.
From Theorem 1, one can pick $\bar n$ sufficiently large such that 
\aln{
C({\bar n}^\alpha) > \frac12 \log {\bar n}^\alpha  = \frac{\alpha}{2} \log \bar n > \rho \log \bar n.
}
Hence, for a Poisson channel with fixed power constraint $\bar n^\alpha$, there exists a code with blocklength $n > \bar n$ and error probability at most $\epsilon$.
Such a code can be used on the PCIP (possibly wasting power) and has the same error probability $\ep$.

\emph{Converse:}
%Conversely, suppose normalized rate $\rho > \alpha/2$ is achievable on the PCIP.
%Fix $\ep > 0$. 
%For some blocklength $n$ there is a code with rate $\rho \log n$ and error probability at most $\ep$ on the PCIP.
%Since this code can use power at most $n^\alpha$, it can 
\end{proof}

%First we claim that, asymptotically, we can remove the integer constraint at the input.
%If we want to transmit $x = u/v$, we can consider picking $L'$ such that $2^{L'} = v 2^L$, using $v$ channel uses (i.e., $v$ strings $z_1,...,z_v$ in $\Sigma^{L'}$), and transmitting $x = 1$ in each of them.
%At the output, the decoder first combines $\tilde y = y[z_v]+...+y[z_v]$ obtaining a channel output distributed as $\Pois(cu)$.
%If the decoder then draws $\tilde y$ random variables independently and uniformly distributed in $\{1,...,v\}$, the total number of counts in each bin will be $\Pois(cu/v)$.
%
%Once we remove the integer constraint at the input, we can also move the parameter $c$ into the power constraint, finally obtaining the Poisson channel
%\aln{
%x[z] \geq 0 \quad \longrightarrow \quad  y[z] \sim \Pois(x[z]),
%}
%with constraint 
%\aln{
%\sum_{z\in \Sigma^L} x[z] \leq cM.
%}
%
%It is not difficult to see that if $M = o(\log M)$, the capacity of the channel goes to $0$ as $2^L \to \infty$, and if 




%We have that 
%$|\set( \{\tilde \y_i \}_{i = 1}^\Nsampled )| =  \| \vf \|_1$,
%and by assumption $\| \vf \|_1 = D = \gamma \M$. 
%
%Then the number of distinct frequency vectors is, by Lemma~\ref{lem:comb}, given by 
%\[
%{ \M^\beta + \M -1 \choose \M^\beta } 
%\]
%Suppose that $\beta \leq 1/2$. Then this term is up to a constant equivalent to
%\[
%{ \M^{\M^\beta} }{ \M^\beta ! }
%\sim
%{ \M^{\M^\beta} }{ \M^{\beta \M \beta}  e^{\M^\beta}},
%\]
%by Stirlings formula.
%Taking the logarithm, we obtain
%\[
%\M^\beta (\log(\M) (1-\beta) + 1)
%\]
%which is larger than the upper bound above, so this argument does not work.. 





==> proof_lemma_noisy_bak.tex <==
% !TEX root = DNA_storage_journal_v2.tex

\section{Proof of Lemma \ref{lem1}}

%\rhcomment{
%We could structure the proof slightly different by first stating the bounds 
%(\ref{eq:bound5}) and (\ref{eq:bound8}), and then showing how with those bounds the proof is concluded. 
%This has the advantage that it becomes clear why those terms a bound together and not individually.
%Then we could have paragraph stating the proofs of the bounds 
%(\ref{eq:bound5}) and (\ref{eq:bound8}). But the current organization also works..
%}


Let $Y^{\len}_1,\ldots, Y^{\len}_\N$ 
be the $\N$ strings observed at the output of the channel.
%; i.e., 
%\aln{
%Y^{\len}_k = Y^{\NL}[k,...,k+\len-1].
%}
First we notice that, since $\N$ is a function of $Y^{\NL}$, we can write 
\al{
H\left(Y^{\NL}\right) & + H\left(S^N|X^{\ML},Y^{\NL}\right) \nonumber \\
%
&= H\left(Y^{\NL},N \right) + H\left(S^N|X^{\ML},Y^{\NL}, N \right) \nonumber \\
%
&= H\left(N \right) + H\left(Y^{\NL} | N \right) + H\left(S^N|X^{\ML},Y^{\NL}, N \right) \nonumber \\
%
&= H(N) + \sum_{n > 0} \Pr(N=n) \left[ H\left(Y^{\NL} | N = n \right) + H\left(S^N|X^{\ML},Y^{\NL}, N =n \right) \right].
}
We show that 
\al{
H\left(Y^{\NL} | N = n \right) + H\left(S^N|X^{\ML},Y^{\NL}, N =n \right) \leq nL + o(ML),
}
and since $H(N) = o(ML)$ and $\Ex[N] = (1-q)M$, the result follows.
%Intuitively, conditioning on $\{N = n\}$ can be thought of as a genie-aided argument 

In order to capture whether we are in the regime of Figure~\ref{fig:points}(a) or (b), we let 
$T$ be the largest subset of $[1:n]$
  so that, for any $i,j \in T$, 
%$\T \subset \Y$ be the largest subset of $\Y$ such that for all $Y_i^{\len}, Y_j^{\len}  \in \T$
$
d_H \left( Y_i^{\len}, Y_j^{\len} \right) \geq \alpha \len,
$
where $d_H$ is the Hamming distance and 
$\alpha > 2p$. % is such that (\ref{eq:condition}) is satisfied.
We assume that in case of ties, an arbitrary tie-breaking rule is used to define $T$ (the actual choice will not be relevant for the proof).
%We also let $T \subseteq [1:\M]$ be the set of indices $i$ such that $Y^{\len}_i \in \T$.
%an indicator vector for $\T$; i.e., a vector such that $T(i) = 1$ if and only if $Y^{\NL}_i \in \T$.
%With a slight abuse of notation we will write $i \in T
%\rhcomment{Here, we could perhaps only define $T$, since in the rest of the proof only $T$ is used..}


Let $\Ex_n$ be the expectation conditioned on $N=n$; i.e.,  $\Ex_n[\cdot] = \Ex[\cdot | N=n]$.
We prove that, given the conditions in Lemma~\ref{lem1}, the following two bounds involving $\Ex_n|T|$ hold:
\begin{subequations}
\begin{align}
\text{(B1)\quad} & H\left(Y^{\NL}| N= n\right) \leq L \Ex_n|T|  % & \quad \quad \quad  
+ (n-\Ex_n|T|)\left( \log \Ex_n|T| + \len H(\alpha) \right) + o(\ML),
 \label{eq:B1}
 \\
\text{(B2)\quad} & H\left(S^N|X^{\ML},Y^{\NL}, N = n\right) \leq 
 n \log n
 % \nonumber \\
%&  \quad \quad \quad 
- \Ex_n|T| \log \Ex_n|T| + o(ML). 
 \label{eq:B2}
%\label{eq:secondterm} 
\end{align}
\end{subequations}
%\al{
%\text{(B1)\quad} & H\left(Y^{\NL}\right) \leq M + L \Ex|T|  \nonumber \\
%& \quad \quad \quad  + (M-\Ex|T|)\left( \log \Ex|T| + \len H(\alpha) \right), \nonumber \\
%% \label{eq:firstterm} \\
%%& H\left(S^N|X^{\ML},Y^{\NL}\right) \leq 
%%1 + \M^{1-\beta D(\delta || p)} \M \log \M \nonumber \\
%%& + M \log M - E|T| \log E|T|,
%\text{(B2)\quad} & H\left(S^N|X^{\ML},Y^{\NL}\right) \leq 
% M \log M \nonumber \\
%&  \quad \quad \quad - \Ex|T| \log \Ex|T| + o(ML). \nonumber 
%%\label{eq:secondterm} 
%}
For large $\Ex_n|T|$, we are typically in the regime of Figure~\ref{fig:points}(a), while Figure~\ref{fig:points}(b) corresponds to the case where $\Ex_n|T|$ is small.
The bounds above capture the tension between the terms $H\left(Y^{\NL}|N=n\right)$ and $H\left(S^N|X^{\ML},Y^{\NL},N=n\right)$ because (B2) is decreasing in $\Ex_n|T|$, while (B1) is increasing in $\Ex_n|T|$ (provided that $\beta(1-H(\alpha)) \geq 1$).
Combining (B1) and (B2),
\al{
& H\left(Y^{\NL}|N=n\right) + H\left(S^N|X^{\ML},Y^{\NL},N=n\right) \nonumber \\
& \quad \leq  \len \Ex_n|T| + (n-\Ex_n|T|)\left( \log \Ex_n|T| + \len H(\alpha) \right) \nonumber \\
& \quad \quad \quad + n \log n - \Ex_n|T| \log \Ex_n|T| + o(\ML) \nonumber \\ 
& \quad = \Ex_n|T| L (1- H(\alpha))  + n \log \Ex_n|T|- 2 \Ex_n|T| \log \Ex_n|T| \nonumber \\
& \quad \quad \quad  + n \len H(\alpha) + n \log n + o(\ML).
\label{eq:boundET} 
}
%\al{
%& H\left(Y^{\NL}\right) + H\left(S^N|X^{\ML},Y^{\NL}\right) \nonumber \\
%& \quad \leq  \len \Ex|T| + (\M-\Ex|T|)\left( \log \Ex|T| + \len H(\alpha) \right) \nonumber \\
%& \quad \quad \quad + \M \log \M - \Ex|T| \log \Ex|T| + o(\ML) \nonumber \\ 
%& \quad = \Ex|T| L (1- H(\alpha))  + \M \log \Ex|T|- 2 \Ex|T| \log \Ex|T| \nonumber \\
%& \quad \quad \quad  + \M \len H(\alpha) + \M \log \M + o(\ML).
%\label{eq:boundET} 
%}
Replacing $\Ex_n|T|$ with $x$ and ignoring the terms in this upper bound that do not involve $x$, we have the expression
%\aln{
%& \beta x \log \M +(\M-x) \log x -x \beta H(\alpha) \log \M - x\log x \\
%& \quad =  \beta(1-H(\alpha)) x \log \M  + \M \log x - 2 x\log x.
%}
\aln{
f(x) \defi  \gamma x  \log \M  + n \log x - 2 x\log x,
}
where we define $\gamma = \beta (1-H(\alpha))$.
For $x > 0$, we have 
\aln{
f'(x) & = \frac{1}{\ln(2)}\left( \gamma \ln \M + \frac{n}{x} - 2\ln x - 2 \right) \\
& > \frac{1}{\ln(2)}\left( \gamma \ln \M - 2\ln x - 2 \right) \\
& = \frac{2}{\ln(2)}\left( \ln \frac{\M^{\gamma/2}}{x} - 1 \right).
}
Hence $f'(x) > 0$ if
%\aln{
%& \log \frac{\M^{\gamma/2}}{x} > 1- \frac{\M}{2x} \\
%\Leftrightarrow \; &  x < 2^{1-\M/2x} M^{\gamma/2}.
%}
\al{
x < e^{-1} M^{\gamma/2}. \label{eq:maxx}
}
We see that, as long as $\gamma > 2$, the right-hand side of (\ref{eq:maxx}) is greater than $M$ for $M$ large enough.
This means that $f(x)$ is increasing for $1 \leq x \leq M$.
Since $\Ex_n|T| \leq n \leq M$, $f$ must attain its maximum at $f(n)$.
%, and must attain its maximum at $f(M)$.
%Notice that $x = \Ex|T| \leq M$.
Therefore, (\ref{eq:boundET}) can be upper-bounded by setting $x = \Ex_n|T| = n$, which yields
\aln{
H\left(Y^{\NL}| N = n\right) & + H\left(S^N |X^{\ML},Y^{\NL},N=n\right) \leq nL + o(\ML).
}
Notice that this holds if, for some $\alpha > 2p$,
\aln{
\gamma = \beta(1-H(\alpha)) > 2 \Leftrightarrow 1 - H(\alpha) - 2/\beta > 0.
}
From the continuity of $H(\cdot)$, such $\alpha$ can be found if \eqref{eq:condition} holds, proving the lemma.
It remains to prove (B1) and (B2).


\subsection{Proof of (B1)}
%We first bound the $H\left(Y^{\NL}\right)$ term as follows:
Since $T$ is a deterministic function of $Y^{\NL}$ and can take at most $2^n$ values, 
\al{
H\left(Y^{\NL}| N = n\right) 
&= H\left(Y^{\NL}, T | N = n \right)  \nonumber \\
&=  H\left( T | N=n \right) +  H\left(Y^{\NL} | T, N=n \right) \nonumber\\
&\leq n + \sum_{t \subseteq [1:n]} \Pr\left( T = t | N = n \right) H\left(Y^{\NL} | T = t, N=n \right). \label{eq:bound3} 
}
Next we notice that, for a given $t$, we can write
\al{
H\left(Y^{\NL} | T = t, N=n \right) & = H\left( [Y^{\len}_i : i \in t] | T = t, N=n \right) \nonumber \\
& \hspace{-8mm} + H\left( [Y^{\len}_i : i \not\in t] | T = t, N=n, [Y^{\len}_i : i \in t] \right). \label{eq:bound4} 
%\\ 
%& \leq |t| L + H\left( \{Y^{\len}_i : i \not\in t\} | T = t, \{Y^{\len}_i : i \in t\} \right)  \\ 
%& \leq |t| L + (\M - |t|) \log\left( |t|  + LH(\alpha) \right),
}
The first term in  (\ref{eq:bound4}) is trivially bounded as 
\aln{
H\left( [Y^{\len}_i : i \in t] | T = t, N=n \right) \leq |t| L.
}
Each of the remaining length-$\len$ strings $Y^{\len}_i$ with $i \notin t$ must be within a distance $\alpha L$ from one of the strings in $[Y^{\len}_i : i \in t]$, from the definition of $T$.
Hence, conditioned on $[Y^{\len}_i : i \in t]$, each of them can only take at most $|t| |B(\alpha L)|$ values, where $B(\alpha L)$ is a Hamming ball of radius $\alpha \len$.
Since $|B(\alpha \len)| \leq 2^{\len H(\alpha)}$ for $\alpha < 1/2$, we bound the second term in (\ref{eq:bound4}) as
\aln{
& H\left( [Y^{\len}_i : i \not\in t] | T = t, N=n, [Y^{\len}_i : i \in t] \right) 
%\\ & \quad \quad \quad \quad 
\leq (n-|t|) \left( \log |t| + \len H(\alpha) \right).
}
Using these bounds back in (\ref{eq:bound3}), we obtain
\al{
\hspace{-2mm} H\left(Y^{\NL} | N=n\right)  \nonumber %\\
% & \; 
& \leq n + \Ex_n  \left[  L |T| + (n-|T|) \left( \log |T| + \len H(\alpha) \right) | N = n \right] + o(\ML) \nonumber \\ & \leq L \Ex_n|T| + (n-\Ex_n|T|)\left( \log \Ex_n|T| + \len H(\alpha) \right) + o(ML),
\label{eq:bound5}
}
where we used the fact that $(n-x) \log x$ is a concave function of $x$ and Jensen's inequality. 

%\rhcomment{Above and thoughout it might be better to write expectation as $\mathbf E$, so it can't be confused with the error pattern $E^{ML}$.}

%The second term in the statement of the lemma can be expanded as
%\aln{
%& H\left(S^N,E^{\ML}|X^{\ML},Y^{\NL}\right) \\
%& = H\left(S^N|X^{\ML},Y^{\NL}\right) + H\left(E^{\ML}|X^{\ML},Y^{\NL},S^N\right).
%}
%Notice that, given $S^N$, one can match each length-$\len$ string in $Y^{\NL}$ to its corresponding length-$\len$ string in $X^{\ML}$, and add them (modulo 2) to obtain the error pattern.
%This implies that $H\left(E^{\ML}|X^{\ML},Y^{\NL},S^N\right) = 0$.

%Finally, we need to bound $H\left(S^N|X^{\ML},Y^{\NL}\right)$.
%Intuitively, given $X^{\ML}$ and $Y^{\NL}$, one can try matching each length-$\len$ string in $Y^{\NL}$ to the closest string in $X^{\ML}$ to try to figure out $S^N$.
%However, this term in general will not be zero (consider, for instance, the case where several of the length-$\len$ strings in $X^{\ML}$ are identical).
%We will bound this term in a way to capture the intuition that, if $\Ex|T|$ is large (i.e., many of the length-$\len$ strings in $Y^{\NL}$ are far from each other), then one can match the strings in the output to the strings in the input more reliably, and $H\left(S^N|X^{\ML},Y^{\NL}\right)$ should be small.

%\vspace{2mm}

%\al{
%\text{(B2)\quad} & H\left(S^N|X^{\ML},Y^{\NL}, N = n\right) \leq 
% n \log n
%- \Ex_n|T| \log \Ex_n|T| + o(ML). \nonumber 
%}
\subsection{Proof of (B2)}
Since $T$ is a deterministic function of $Y^{\NL}$,
\al{
& H\left(S^N|X^{\ML},Y^{\NL}, N = n\right) = H\left(S^N|X^{\ML},Y^{\NL}, T, N = n\right) \nonumber \\
& =  \sum_{t \subseteq [1:n]} \Pr\left( T = t | N = n\right) H\left(S^N|X^{\ML},Y^{\NL}, T = t, N = n\right) \nonumber \\
& \leq  \sum_{t \subseteq [1:n]} \Pr\left( T = t | N = n\right) \sum_{i=1}^n H\left(S(i)|X^{\ML},Y^{\NL}, T = t , N = n\right). \label{eq:bound6} 
}
Next we notice that the probability that $\delta \len$ or more errors occur in a single length-$\len$ string, for $\delta > p$, is at most $2^{-\len D(\delta \| p)}$ by the Chernoff bound (where $D(\cdot \| \cdot)$ is the binary KL divergence).
If we let $\E_i$ be the event that $d_H\left( X_{S(i)}^\len, Y_i^\len \right) \geq \delta L$, then we have
\aln{
\Pr(\E_i) \leq 2^{-\len D(\delta \| p)} = \M^{-\beta D(\delta \| p)}.
}
The conditional entropy term in (\ref{eq:bound6}) is upper bounded by
%
% Technically, H(1_E) should be H(1_E|T=t), but then it won't fit
%
\al{
& H\left(S(i), \one_{\E_i}|X^{\ML},Y^{\NL}, T = t, N = n\right) \nonumber \\
& \quad  \leq H(\one_{\E_i}| T=t,N = n) + \Pr(\E_i | T = t, N = n) H\left(S(i)|X^{\ML},Y^{\NL}, T = t, N = n, \E_i \right) \nonumber \\
& \quad \quad \quad + \Pr(\bar\E_i | T = t, N = n) H\left(S(i)|X^{\ML},Y^{\NL}, T = t, N = n, \bar\E_i \right) \nonumber \\
& \quad \leq 1 + \Pr(\E_i | T = t, N = n) \log \M \nonumber \\
& \quad \quad \quad + H\left(S(i)|X^{\ML},Y^{\NL}, T = t, N = n, \bar\E_i \right)
%& \quad \leq H\left(S^N|X^{\ML},Y^{\NL}, T = t, \bar\E \right) + o(\ML),
\label{eq:bound7}
}
The final step is to bound the conditional entropy term in (\ref{eq:bound7}), for the case where $i \in t$.
%In the case where $i \notin t$, we will trivially bound it by $\log M$.
%So consider the case where $i \in t$, and let us 
Set $\delta = \alpha/2$. 
Conditioned on $\bar\E_i$, $d_H\left( X_{S(i)}^\len, Y_{i}^\len \right) < \alpha \len/2$.
Moreover, conditioned on $T=t$, for any $j \in t - \{i\}$, $d_H\left( Y_i^\len, Y_j^\len \right) \geq \alpha \len$.
%there are $|t|-1$ length-$\len$ output strings $\{Y_j^\len : j \in t, j \ne i\}$ that are all at distance at least $\alpha L$ from $Y_i$.
For $i \in t$, we define the set 
%
%
%%none of the original strings in $X^{\ML}$ are more than a distance $\delta \len$ from their corresponding string in $Y^{\NL}$.
%
%
%%Then, each of the strings in $X^{\ML}$ corresponding to the output strings in $t$ is within a distance less than $\len \alpha/2$ from its output string which, in turn is at a distance of at least $\alpha L$ from $|t|-1$ other strings.
%
%
%
%
%Then, each string $X_i^\len$ such that $S^{-1}(i) \in t$ is within a distance less than $\len \alpha/2$ from $Y_{S^{-1}(i)}^\len$, which in turn is at a distance of at least $\alpha L$ from $|t|-1$ other strings.
%For each $i \in t$, we let 
\aln{
A_i = \{ j \st Y^{\len}_i \text{ is the closest output string in $t$ to }X^{\len}_j \}.
}
Notice that $A_i$, $i\in t$, forms a partition of $[1:M]$.
We claim that, if $i \in t$, $S(i)$ must be in $A_i$.
To see this notice that, for any $k \in t$, $k \ne i$, we have
%Otherwise, $X_{S(i)}^{\len}$ would be closer to another string $Y_k^\len$ with $k \in t$ than to $Y_i^{\len}$.
%But this is impossible since 
\aln{
\alpha \len & \leq d_H \left( Y_i^{\len}, Y_k^{\len} \right) \\
& \leq d_H \left( X_{S(i)}^{\len}, Y_i^{\len} \right) + d_H \left( X_{S(i)}^{\len}, Y_k^{\len} \right)  \\
& < \alpha \len/2 + d_H \left( X_{S(i)}^{\len}, Y_k^{\len} \right),
}
implying that $d_H \left( X_{S(i)}^{\len}, Y_k^{\len} \right) > \alpha \len/2 \geq d_H \left( X_{S(i)}^{\len}, Y_i^{\len} \right)$, and thus $S(i) \in A_i$.
%
%$d_H \left( Y_i^{\len}, Y_j^{\len} \right) \geq \alpha \len$ and 
%$d_H \left( X_{S(i)}^{\len}, Y_j^{\len} \right) < \alpha \len /2$
Therefore, $S(i)$ for each output string $Y^{\len}_i$ with $i \in t$, can take at most $|A_i|$ values.
%So we can bound the entropy term in (\ref{eq:bound7}) as
Hence we have
%\aln{
%& H\left(S(i)|X^{\ML},Y^{\NL}, T = t, \bar\E_i \right) \leq \log |A_i|,
%} % \label{eq:boundAi}
%and 
\al{
& \sum_{i=1}^n H\left(S(i)|X^{\ML},Y^{\NL}, T = t, N = n, \bar\E_i \right) \nonumber \\
%& \quad \quad \quad \leq \sum_{i \not\in t}H(S(i)) + \sum_{i \in t} \log |A_i| \nonumber \\
& \quad \quad \quad \leq \sum_{i \not\in t} \log M + \sum_{i \in t} \log |A_i| \nonumber \\
& \quad \quad \quad = (n-|t|) \log M + \sum_{i \in t} \log |A_i| \nonumber \\
& \quad \quad \quad \leq (n-|t|) \log M +|t| \log (M/|t|) \nonumber \\
& \quad \quad \quad = n \log M - |t| \log |t|, \label{eq:boundAi}
}
where the last inequality follows because $\sum_{i \in t} |A_i| = M$, and the sum is maximized by $|A_i| = \M/|t|$.
Combining (\ref{eq:bound6}), (\ref{eq:bound7}), and (\ref{eq:boundAi}), we obtain
\al{
& H\left(S^N|X^{\ML},Y^{\NL}, N=n\right)  \nonumber \\
& \quad  \leq  \sum_{i=1}^n \sum_{t \subseteq [1:n]} \Pr\left( T = t | N=n \right)\left[ 1 + \Pr(\E_i | T = t, N=n) \log \M  \right] \nonumber \\
& \quad  \;\; +  \sum_{t \subseteq [1:n]} \Pr\left( T = t | N=n\right) \sum_{i=1}^n H\left(S(i)|X^{\ML},Y^{\NL}, T = t, N=n, \bar \E_i \right) \nonumber \\
& \quad  =  n + \log M\sum_{i=1}^n \Pr(\E_i | N=n) + n \log M - \Ex_n\left[|T| \log |T|\right] \nonumber \\
& \quad  \leq  n + M \log M\sum_{i=1}^n \Pr(\E_i | N=n) + n \log M - \Ex_n\left[|T| \log |T|\right] \nonumber \\
& \quad  \leq  n + n \log M (1+M^{-\beta D(\delta \| p)} ) - \Ex_n |T| \log \Ex_n |T| \nonumber
%\label{eq:bound8} 
}
%
%
%
%\aln{
%& H\left(S(i)|X^{\ML},Y^{\NL}, T = t, \bar\E_i \right) \nonumber \\
%& \quad \quad \quad \leq \sum_{i \not\in t}H(S(i)) + \sum_{i \in t} \log |A_i| \nonumber \\
%& \quad \quad \quad \leq (M-|t|) \log M + \sum_{i \in t} \log |A_i|.
%}
%%\aln{
%%& H\left(S^N|X^{\ML},Y^{\NL}, T = t, \bar\E \right)  \nonumber \\
%%& \quad \quad \quad \leq \sum_{i \not\in t}H(S(i)) + \sum_{i \in t} \log |A_i| \nonumber \\
%%& \quad \quad \quad \leq (M-|t|) \log M + \sum_{i \in t} \log |A_i|.
%%}
%Since $\sum_{i \in t} |A_i| = M$, the sum is maximized by $|A_i| = \M/|t|$, and we have
%\aln{
%& H\left(S^N|X^{\ML},Y^{\NL}, T = t, \bar\E \right)  \nonumber \\
%& \quad \quad \quad \leq (M-|t|) \log M +|t| \log (M/|t|) \nonumber \\
%& \quad \quad \quad = M \log M - |t| \log |t|.
%}
%Therefore, from (\ref{eq:bound6}) and (\ref{eq:bound7}), we obtain
%\al{
%H\left(S^N|X^{\ML},Y^{\NL}\right) & \leq 1 + \Pr(\E) \M \log \M \nonumber \\
%& \quad \; \; \;  + M \log M - \Ex|T| \log \Ex|T| \nonumber \\
%& \leq 1 + \M^{1-\beta D(\delta || p)} \M \log \M \nonumber \\
%& \quad \; \; \;  + M \log M - \Ex|T| \log \Ex|T|,
%\label{eq:bound8} 
%}
where, in the last step we used the fact that $\E_i$ is indepedent of $N=n$, and Jensen's inequality.
Since $ \M^{-\beta D(\delta || p)} \to 0$ as $\M \to \infty$,
$\M^{-\beta D(\delta || p)} \M \log \M = o(\ML)$, concluding the proof. 
 

 
  
%    , we now combine (\ref{eq:bound5}) and (\ref{eq:bound8}) to obtain 
%\al{
%& H\left(Y^{\NL}\right) + H\left(S^N,Z^{\ML}|X^{\ML},Y^{\NL}\right) \leq \nonumber \\
%& \quad  \len \Ex|T| + (\M-\Ex|T|)\left( \log \Ex|T| + \len H(\alpha) \right) \nonumber \\
%& \quad + \M \log \M - \Ex|T| \log \Ex|T| + o(\ML). \label{eq:bound9} 
%}
%Replacing $\Ex|T|$ with $x$ and ignoring the terms in this upper bound that do not involve $x$, we have the expression
%\aln{
%& \beta x \log \M +(\M-x) \log x -x \beta H(\alpha) \log \M - x\log x \\
%& \quad =  \beta(1-H(\alpha)) x \log \M  + \M \log x - 2 x\log x.
%}
%Let $f(x)$ be the above expression, and let $\gamma = \beta(1-H(\alpha))$.
%For $x > 0$, we have 
%\aln{
%f'(x) & = \frac{1}{\ln(2)}\left( \gamma \log \M + \frac{M}{x} - 2\log x - 2 \right) \\
%& > \frac{1}{\ln(2)}\left( \gamma \log \M - 2\log x - 2 \right) \\
%& = \frac{2}{\ln(2)}\left( \log \frac{\M^{\gamma/2}}{x} - 1 \right).
%}
%Hence $f'(x) > 0$ if
%%\aln{
%%& \log \frac{\M^{\gamma/2}}{x} > 1- \frac{\M}{2x} \\
%%\Leftrightarrow \; &  x < 2^{1-\M/2x} M^{\gamma/2}.
%%}
%\aln{
%x < \frac12 M^{\gamma/2}.
%}
%We see that, as long as $\gamma > 2$, the right-hand side is greater than $M$ for $M$ large enough.
%This means that $f(x)$ is increasing for $1 \leq x \leq M$, and must attain its maximum at $f(M)$.
%Therefore, (\ref{eq:bound9}) can be upper-bounded by setting $x = \Ex|T| = M$, which yields
%\aln{
%H\left(Y^{\NL}\right) + H\left(S^N,Z^{\ML}|X^{\ML},Y^{\NL}\right) \leq \ML + o(\ML).
%}
%This concludes the proof of Lemma \ref{lem1}.


%\aln{
%& \beta x \log M +(M-x) (\log x + \beta H(\alpha) \log M) + M \log M - x\log x \\
%& \quad = x \left( \beta (1-H(\alpha)) \log M - 2 \log x \right) + M \log x + M \log M (1 + \beta H(\alpha))
%}






